"What's This?" -- Learning to Segment Unknown Objects from Manipulation Sequences

We present a novel framework for self-supervised grasped object segmentation with a robotic manipulator. Our method successively learns an agnostic foreground segmentation followed by a distinction between manipulator and object solely by observing the motion between consecutive RGB frames. In contrast to previous approaches, we propose a single, end-to-end trainable architecture which jointly incorporates motion cues and semantic knowledge. Furthermore, while the motion of the manipulator and the object are substantial cues for our algorithm, we present means to robustly deal with distraction objects moving in the background, as well as with completely static scenes. Our method neither depends on any visual registration of a kinematic robot or 3D object models, nor on precise hand-eye calibration or any additional sensor data. By extensive experimental evaluation we demonstrate the superiority of our framework and provide detailed insights on its capability of dealing with the aforementioned extreme cases of motion. We also show that training a semantic segmentation network with the automatically labeled data achieves results on par with manually annotated training data. Code and pretrained model are available at https://github.com/DLR-RM/DistinctNet.

==> experiments.tex <==
%\begin{table*}[!ht]
%	\centering
%	\caption[Quantitative results]{Quantitative comparison of our method compared to three baseline approaches and \cite{florence2019self}; for a better overview we first list the joint objects. The right-most column shows results on semantic segmentation in a table top scene, where we use our automatically generated object masks as training data. Numbers in \textbf{bold} denote the best results on object-in-gripper segmentation.}
%	\vspace*{1mm}
%	\resizebox{0.9\textwidth}{!}{
%		\input{../tables/quant_results}}
%	\label{tab:quant_results}
%\end{table*}


In this section we evaluate the performance of our method on self-supervised grasped object segmentation. 
We further provide insights on the model's capability to deal with moving background objects and static input frames.
We continue by exploring different architectural settings to explain our network design choices.
Finally we show that the generated masks show equal or better performance for the task of semantic segmentation from scenes in comparison to a subset of ground truth annotations.

%For a full quantitative comparison under use of \emph{mean Intersection over Union} we manually create ground truth annotations for a subset of object and robot arms (15\% per object; object and robot poses are identical across object categories).
%The main metric of evaluation is the \emph{mean Intersection over Union} between ground truth robot and object annotations and our predictions.

\subsection{Evaluation of Self-Supervised Object Segmentation}

We quantitatively evaluate our method in Tab. \ref{tab:quant_results} and report the \emph{mean Intersection over Union} (\emph{mIoU}) for all objects as well as robot arm, moving foreground and background.
Adding the gripper as separate semantic label (\mbox{Sec. \ref{sec:dataset_robobj}}) increases overall object mIoU by one percent point.

DistinctNet generates strong segmentation masks (left part of Fig. \ref{fig:qual_results}), and we outperform recent self-supervised approaches with similar weak constraints on the setup by a large margin.
Despite not using camera calibration, manipulator key point registration and additional depth data like~\cite{florence_robot-supervised_2020} we still reach similar performance on a joint subset of objects (82.72\% vs. 84.61\% mIoU).
%Furthermore, we come close to a recent framework by Florence~et~al.~\cite{florence_robot-supervised_2020} which exploits camera calibration, robot manipulator key point registration and additional depth data.
%We achieve 82.72\% mIoU on a joint subset of objects compared to their respectable performance of 84.61\%.
%On the joint subset of objects 

Nevertheless, some object views are quite challenging to our approach (middle part of Fig. \ref{fig:qual_results}), and a particularly outstanding item is the \emph{037\_scissors}. 
We hypothesize that due to the thin shape of the object the network finds it difficult to establish correspondences between two consecutive frames and identify it as moving object.
This would also explain the superior performance of \cite{florence_robot-supervised_2020} on this item, as their approach does not rely on identification by motion.
%While semantic finetuning visually improves moving foreground segmentation (see right part of Fig. \ref{fig:qual_results}), the \emph{scissors} perform by far worst across all objects for our method.


We concurrently observe that fine-tuning on semantics improves moving foreground extraction (right part of Fig.~\ref{fig:qual_results}):
Initially, DistinctNet segments joint robot-object masks from our test set with a mIoU score of 86.56\%. As reported in Tab. \ref{tab:quant_results} this increases by roughly six percent points after fine-tuning, indicating that semantic knowledge (albeit here merely in the form of background, object and manipulator) is important for segmentation from motion, which is in line with previous research (Sec.~\ref{sec:rl_combination}).
%We conclude that semantic knowledge is important for motion segmentation.
Furthermore, while we hypothesize that the correlation operation itself ensures strong generalization from synthetic to real data, the semantic fine-tuning might also be helpful for bridging a remaining sim2real gap.

\begin{figure*}[!ht]
	\vspace{4mm}
	\centering
	\captionsetup{width=\linewidth}
	\includegraphics[width=0.9\linewidth]{../figures/qual_results/qual_results_res.png}
	\caption{DistinctNet generates semantic annotations of a moving manipulator with a grasped object and optional other classes like the gripper (left images);
		Some items are particularly challenging because of similar color to surroundings or due to their shape (middle images);
		Fine-tuning on semantics increases performance on moving foreground extraction (right images).}
	\label{fig:qual_results}
\end{figure*}%

\begin{table}[!hb]
	\centering
	\caption[Comparison to Baselines]{Mean IoU ([\%]) of our method compared to change detection and two recent approaches from literature.
%		 (\cite{florence_robot-supervised_2020, boerdijk_self-supervised_2020}). 
\emph{Ours+G.} denotes predictions with an additional gripper output channel.
Numbers in \textbf{bold} depict best results.}
	\vspace*{1mm}
	\resizebox{0.95\columnwidth}{!}{
		\input{../tables/quant_results_baseline}}
	\label{tab:quant_results}
\end{table}

\subsection{Extreme Cases of Motion}
Our method typically relies on motion of manipulator and object.
Nevertheless, small modifications to our framework allow to deal with challenging scenarios such as moving background items or no observable motion at all.

%However, in practice there might be cases where either parts of the background move as well, or the motion of manipulator and object drops below an identifiable minimum. 
%The architecture of DiffNet allows to handle such challenging scenarios.

\subsubsection{Dealing with Non-Static Background Objects}
\label{sec:garbage}
We can efficiently learn the presence of other moving objects by treating them as a new semantic class and adding another output channel to our network during semantic fine-tuning.
%Consequently, during semantic fine-tuning we simply add another output channel denoting other moving objects.
We emulate random background object motion by pasting additional objects onto our training data with different random spatial positions between consecutive frames.
After training, DistinctNet successfully differentiates a grasped object from other moving distractor items, as visualized in Fig. \ref{fig:moving_background}. Thereby, the overall object mIoU is merely reduced by 3\% due to mismatches between the grasped item and an object moving in the background.
This makes our approach more versatile in practical applications than our previous work, where every moving pixel not identified as manipulator is automatically classified as grasped object.
%We believe that this is an essential step towards practical applicability of our method. 



\begin{figure*}[!ht]
	\centering
	%1357
	\subfloat[][Image 1]{\includegraphics[width=0.18\textwidth]{../figures/moving_garbage/im1.png}} %was 0-19
	\enskip
	\subfloat[][Image 2]{\includegraphics[width=0.18\textwidth]{../figures/moving_garbage/im2.png}}
	\enskip
	\subfloat[][Prediction]{\includegraphics[width=0.18\textwidth]{../figures/moving_garbage/banana_masked_red.png}}
	\enskip
	\subfloat[][Object Heatmap]{\includegraphics[width=0.18\textwidth]{../figures/moving_garbage/heatmap.png}}	
	\enskip
	\subfloat[][Thresholded Flow]{\includegraphics[width=0.18\textwidth]{../figures/moving_garbage/raft_sintel_binary.png}}
%	\enskip
%	\subfloat[][Gripper Mask]{\includegraphics[width=0.155\textwidth]{../figures/moving_garbage/image905.png}}
	
	\caption[Background motion]{Augmented moving background objects between two consecutive frames (a, b); Our network can directly separate moving foreground into grasped object (green), manipulator (orange) and other moving objects (red) (c); We sample 1,000 different objects on random positions on the image and visualize whether the item is identified as grasped object or belongs to moving background objects (d); While thresholded optical flow successfully segments moving foreground the binary prediction requires additional reasoning to differentiate objects into manipulator, object and distractor (e).}
	
	\label{fig:moving_background}
\end{figure*}


\subsubsection{Dealing with Motion Stops}
\label{sec:extreme_stop}
%In contrast to the above, manipulator and / or object might also come to a rest for a short period of time.
To alleviate the constant dependency on motion for successful prediction we propose to add a \emph{ConvLSTM} layer after the ASPP module and replace every \emph{Conv2d} layer in the decoder with the respective recurrent counterpart (see also Fig. \ref{fig:arch}).
Whenever both input images are alike (i.e., no observable motion between frames), the network still estimates manipulator and object given the memorized predictions of previous frames.
We quantitatively analyze the decrease in mIoU after a motion stop in Fig. \ref{fig:recurrent}.
%We quantitatively analyze this behavior by feeding ten consecutive frames followed by equal input pairs to emulate a motion stop.
%Fig. \ref{fig:recurrent} visualizes the mean and variance across all objects of the mIoU drop with respect to the initial values.
%Mean and variance of the mIoU drop with respect to the initial values are visualized in 

%and plot mean and variance of the mIoU drop in Fig. \ref{fig:recurrent}.


\begin{figure}[!b]
	\centering
	\captionsetup{width=\linewidth}
	\includegraphics[width=0.8\linewidth]{../figures/recurrent/recurrent_final.png}
	\caption{
		After ten consecutive frames we simulate a motion stop by feeding equal input pairs to the network
%		We feed the network ten consecutive frames and  followed by equal input pairs to emulate motion stop 
		(t=0 denotes the last moving input pair). 
		We repeat this five times per object, and plot mean and variance of the IoU relative to the point where motion last occurred across all objects.
		On average, DistinctNet still predicts 80\% of the initial segmentation mask after 20 static frames.}
	\label{fig:recurrent}
\end{figure}%

% method typically relies on motion of manipulator and object.

\subsection{Ablation Study}
\label{sec:ablation}
We experiment with various placements of the correlation layer and a co-attention operation \cite{lu_hierarchical_2016, lu_see_2019} to explain our architectural design choices. 
%To verify our architectural choice of placing the correlation layer after the second ResNet block we explore several other possible settings.
%We further experiment with a co-attention layer  which is usually placed after the ASPP module.
In \cite{lu_see_2019} co-attention is performed after the ASPP module, and we add an experiment with the co-attention block placed at the position of the best-performing correlation setting for fair comparison.
In Tab.~\ref{tab:architecture_ablation} we list the mIoU for the task of agnostic segmentation from motion (Sec. \ref{sec:moving_obj_seg}) with our synthetic validation set \mbox{(Sec. \ref{sec:dataset_fg})} and joint robot-object masks as test~set~\mbox{(Sec. \ref{sec:dataset_test})} after five epochs of training.
We further show the number of parameters in million. 
For the inference estimate we average ten forward passes (single batch size, including image pre-processing) in evaluation mode.
Our proposed setting of employing a correlation layer after the second ResNet block results in best performance on both data splits, while simultaneously being substantially faster than all other settings.
We hypothesize that the comparatively bad performance of the co-attention layer stems from strong augmentations on both images.


\begin{table}[!t]
	\centering
	\caption[Quantitative results]{Architectural ablation study on different merge layers and positions. Our setting (\textbf{bold}) results in best performance for moving foreground segmentation in terms of mIoU on validation and test set while operating at~\texttildelow14~Hz.}
	\vspace*{1mm}
	\resizebox{\columnwidth}{!}{
		\input{../tables/architecture_ablation}}
	\begin{tabular}{l}
	\footnotesize{*Here, segmentation maps for both inputs are predicted as per \cite{lu_see_2019}.}
	\end{tabular}

	\label{tab:architecture_ablation}
\end{table}

%\begin{table}[!ht]
%	\centering
%	\caption[Quantitative results]{Ablation Study.}
%	\vspace*{1mm}
%	\resizebox{\columnwidth}{!}{
%		\input{../tables/training_ablation}}
%	\label{tab:training_ablation}
%\end{table}

%\subsection{Downstream Tasks}

%In this section we show that the predicted YCB object masks (301 views per object) perform equally well or better compared to ground truth annotations (45 views per object) as training data for semantic segmentation or for photogrammetric 3D reconstruction.

%We exemplary show that the generated masks are well suited as training data for semantic segmentation.

%In our previous work we showed that the generated masks are well suited as training data for semantic segmentation, and can also be used for 3D reconstruction of texture-rich objects.
%In this paper we provide insights on the performance of these downstream tasks while comparing to ground truth annotations (45 of 301 masks per object) which serve as upper baseline.

\subsection{Semantic Segmentation as Downstream Task}
We evaluate the quality of our automatically generated object masks by employing them as training data for semantic segmentation.
Specifically, we are interested in the performance of these masks in contrast to manually annotated object masks (i.e., the ground truth annotations we compare to in Tab. \ref{tab:quant_results}), and the improvements to our previous work.

Diverse training data (50,000 images) is generated by pasting object masks
with random scale and translation on MS~COCO~\cite{lin_microsoft_2015} backgrounds. 
We train a standard DeepLabv3+ \cite{chen_encoder-decoder_2018} with the same settings as for moving object segmentation (Sec. \ref{sec:implementation_details}) and compare ground truth and predicted masks on images of STIOS \cite{durner2021unknown}
%the DLR TableTop Dataset\footnote{To be released.} 
in Tab. \ref{tab:semseg}.
We visualize exemplary results in Fig. \ref{fig:semseg}.

For equal views across all masks the ground truth annotations represent an upper border, and we perform superior to masks generated by \cite{boerdijk_self-supervised_2020} due to better initial \mbox{quality (see Tab. \ref{tab:quant_results})}.
Remarkably, the network benefits from many additional views, and employing all object views segmented by our approach as training data performs better than the smaller subset of ground truth annotations.
Note that while there is no experiment with 301 ground truth masks per object we expect an analogous upper bound.% as with 45 masks.

\begin{figure}[!b]
	\centering
	\captionsetup{width=\linewidth}
	\includegraphics[width=0.8\linewidth]{../figures/semseg/semseg_res.png}
	\caption{
		Qualitative results from our semantic segmentation from scenes (best viewed magnified). We add bounding boxes to denote the class labels of the respective annotations.}
	\label{fig:semseg}
\end{figure}%



\begin{table}[t]
	\centering
	\caption[Quantitative results]{Mean IoU on segmentation from tabletop scenes. Training data are a subset (45) or all (301) masks per grasped object. We use our generated annotations, predictions from~\cite{boerdijk_self-supervised_2020} as well as ground truth annotations.}
	\vspace*{1mm}
	\resizebox{0.7\columnwidth}{!}{
		\input{../tables/semseg_mean}}
	\label{tab:semseg}
\end{table}

%\subsubsection{3D Reconstruction}
%We exemplary show that all predicted views result in a more completed reconstruction than the subset of ground truth masks in Fig. \ref{fig:3drec} for the \emph{003\_cracker\_box}.
%For reconstruction we use Agisoft Metashape \todo{cite}.
%%For 3D reconstruction we use Agisoft Metashape \todo{cite}. 
%%Interestingly, as indicating in Fig. \ref{fig:3drec}, 45 ground truth views result in an incomplete reconstruction. 
%%While all 301 predicted masks might contain gripper or background parts, or under-segmented views they yield a qualitatively higher reconstruction.
%
%\begin{figure}[!t]
%	\centering
%	\subfloat[][45 GT masks]{\includegraphics[width=0.15\textwidth]{../figures/3drec/gt.png}}
%%	\enskip
%	\subfloat[][301 Pred. masks]{\includegraphics[width=0.15\textwidth]{../figures/3drec/pred.png}}
%%	\enskip
%	\subfloat[][Original]{\includegraphics[width=0.15\textwidth]{../figures/3drec/orig.png}}
%	\caption{
%		Qualitative differences in 3D reconstruction of the \emph{003\_cracker\_box} from 45 ground truth frames (left) and 301 predicted frames (middle) compared with the original model (right).}
%	\label{fig:3drec}
%\end{figure}%
%
%
%%\begin{table}[!ht]
%%	\centering
%%	\caption[Comparison to Baselines]{Quantitative comparison of our method compared to three baseline approaches and \cite{florence2019self}; for a better overview we first list the joint objects. The right-most column shows results on semantic segmentation in a table top scene, where we use our automatically generated object masks as training data. Numbers in \textbf{bold} denote the best results on object-in-gripper segmentation.}
%%	\vspace*{1mm}
%%	\resizebox{\columnwidth}{!}{
%%		\input{../tables/ablation_raft_models}}
%%	\label{tab:ablation_raft_models}
%%\end{table}
%


==> introduction.tex <==
One of the key functionalities for any robotic manipulation system is
the ability to accurately determine the location of the object(s) to
be manipulated. To do this, most current systems employ computer
vision techniques, where the aim is to find the pixels that correspond
to the target object within a camera image taken from the scene. This
is called \emph{object segmentation}, and it is an important
prerequisite for a large number of downstream tasks such as object
pose estimation, 3D reconstruction, or grasp detection. In general,
object segmentation can be treated in two different ways, depending on
whether a representation of the object is given beforehand, for example in
form of a 3D model. If such a model exists, the segmentation problem
is significantly easier, because the model can be used to guide the
search, e.g. by training an object detector. Unfortuntaley, it is also
the less common case, because 3D models are often not available.

\begin{figure}[!t]
	\centering \captionsetup{width=\linewidth} \includegraphics[width=0.9\linewidth]{../figures/cover/cover_final_res.png} \caption{Our
	approach first learns to segment objects that move in the
	foreground (top). Then, we use fine-tuning to learn a
	segmentation between the manipulator and the unknown object
	(center). Furthermore, our model can distinguish moving
	background objects (bottom left) and support
	downstream tasks such as semantic segmentation (bottom right).  \label{fig:cover}}
%	\caption{We learn agnostic moving object segmentation from synthetic RGB data. 
%	Our model can generate training data for unknown object segmentation from robotic motions and be finetuned on this task.
%	Our approach can robustly deal with background object motion, and the automatically generated masks can be used as training data for e.g. semantic segmentation (best viewed magnified; for object classes we visualize bounding boxes).
%	\label{fig:cover}}
\end{figure}%



Therefore, in this work we address segmentation of unknown objects,
where the only cue we rely on is the change of pixels that occurs when
moving the object in front of the camera. This can either be done by
pushing the object on a
table \cite{Fitzpatrick2003GroundingVT,schiebener_physical_2014,pathak_learning_2018,deng2020self}
or by holding it with a gripper and moving it with the manipulator. We
follow the latter approach, because then the object can be seen from
all sides, including from the bottom. We also
employ \emph{self-supervised} object segmentation, i.e. for segmentation we neither
require a kinematic model of the manipulator nor an intrinsic or
extrinsic calibration of the camera. This makes our approach
particularly versatile and easy to use. Also, in contrast to existing
works, we do not perform a two-step process where first a representation of the
manipulator is learned, before the actual object segmentation can be
done. Instead, we propose an end-to-end learning scheme where the
segmentation of both the manipulator and the object are learned
simultaneously. This has the major advantage that information can be
shared between the two tasks, and hyperparameter tuning or post
processing are not required. Furthermore, 
%by adding a specific head in
%the architecture, 
our approach is able to distinguish between objects
that are actively moved by the manipulator and those that move in the
background (see Fig.~\ref{fig:cover}). Finally, our architecture
provides means to segment the object even in cases where no motion is
observed for a small number of frames. As we will show experimentally,
our approach outperforms previous self-supervised methods, and it even
competes with techniques that rely on hand-eye calibration and additional depth data.

%accurate ground-truth
%annotations.




%\todo{say something about the necessity of real world training data, and the tedious problem of labeling}

%Accurate object segmentation is essential for successful recognition, interpretation and interaction within a robot's environment.
%While neural networks excel in many vision-related tasks~\cite{wu2019detectron2}, their inherent data-driven characteristic limits applicability within real world robotic environments.

%A major reason therefore is In ever-changing environments robots concurrently perceive novel, unknown instances

%A major reason therefore is a robot's concurrent encounter of unknown objects.
% in ever-changing environments.
% which a robot typically encounters in unstructured environments.
%For successful perception and interaction of such novel instances the creation of training data 
%for neural networks 
%is usually inevitable - let it be in the form of real-world sensor annotations~\cite{maninis2018dextr}, or by 3D model generation for synthetic data creation, domain randomization or domain adaptation (e.g.~\cite{hodan_photorealistic_2019, ferrari_implicit_2018}).
%Nevertheless, the enormous expenditure of time and human involvement for such tasks makes this in practice often infeasible~\cite{maji_large_nodate}.


%such labeled sensor data is not readily available


%Neural networks excel at many vision-based tasks \cite{wu2019detectron2}, but typically require tons of carefully labeled training data.
%Yet, due to concurrent perception of novel, unseen instances such labeled sensor data is not readily available, but would require tedious manual labeling.

%While there has been strong progress 

%Fine-tuning on novel class instances delivers promising results, but still requires manual annotations.





%- neural nets excel, but require lots of data
%- synthetic / domain randomization / domain adaptation: promising, but require 3d models

%Neural networks typically excel at such tasks but often require a tremendous amount of manually labeled data. \todo{cite, say that there are other ways but usually real world data yields best performance}

%To this end, self-supervised object segmentation presents an elegant way to 
%automatically create real world sensor data annotations on a large scale.
%It is typically formulated as a two-step process consisting of (1) reasoning about the manipulator and (2) separating the then known manipulator from any unknown object. 
%Usually, a foreground estimator is employed for the first task, and with the resulting manipulator masks a representation of the grasping arm is learned.
%Whenever grasping an unknown object the same foreground predictor is used to obtain a joint object-manipulator mask. Finally, the learned manipulator representation is used to separate the foreground into object and grasping arm.

%Previous work successfully follow this paradigm with smart integration of robot arm kinematics, depth data or motion. 
%Nevertheless, a major caveat of all approaches is that the foreground estimation and the separation in manipulator and object is always formulated as two standalone tasks. 
%Consequently, end-to-end optimization is usually difficult due to non-differentiable operations or large building blocks. 
%More importantly, information between the two tasks is only shared to a certain extend, if at all. 
%As a result, current methods require careful tuning of hyperparameters, specific post-processing, integration of kinematic information, additional sensor data or testing backgrounds to produce satisfactory results.

%We believe that these constraints limit current applicability of self-supervised data generation pipelines, and propose a novel framework which addresses these issues.

%First, we design a single, end-to-end trainable architecture that is capable of efficiently estimating moving foreground, and simultaneously allows for being fine-tuned on separating the moving parts into manipulator and object from single RGB camera streams only.

%We show that our joint formulation yields strong segmentation performance.

%Second, while we use motion as main premise our approach can robustly deal with extreme cases in the form of additional moving background objects or scenarios where object and manipulator come to a halt.

%Third, we only use synthetic data or labels generated by self-supervision during training to ensure universal applicability of our framework.
%Our method is not constrained on precise hand-eye calibration, and our pre-trained motion estimator can be fine-tuned irrespective of manipulator or testing environment. 
%The generated masks do not require any post-processing.

%With extensive experimental evaluation we show that our framework produces strong segmentation results and outperforms several baselines and approaches from literature.
%The self-supervised generated masks perform en par compared to ground truth annotations as training data for semantic segmentation. \todo{rephrase}

%\todo{say that its named diffnet?}

%\todo{cover figure: result of quantitative segmentation, result of hand + object, semantic segmentation}



==> method.tex <==
%The only requirement for our self-supervised segmentation is motion of manipulator and object, and a static background. We therefore design an architecture that can jointly be used for moving object segmentation and then fine-tuned on separating object from manipulator, and will explain this in detail here.

%\todo{some sentences about this section}
%also say something about the general pipeline - i.e., segment moving objects, fine tune this with pasted robot arms following \todo{florence, ours}

%A major contribution of this work is to simultaneously optimize moving foreground and object-manipulator differentiation.



We modify a standard DeepLabv3+~\cite{chen_encoder-decoder_2018} with a \mbox{ResNet-50}~\cite{he_deep_2015} backbone which has proven to be successful for many semantic segmentation applications. 
In the following we refer to our network as \emph{DistinctNet}, as it allows to (1) distinguish moving foreground from static background as well as (2) semantically differentiate objects.
We now further explain our modifications that let us predict moving foreground and allow for fine-tuning on robot-object segmentation.
For an overview of our pipeline please see~Fig.~\ref{fig:arch}.
%- problem formulation (or in introduction?)
%- architecture + training details
%- learning foreground segmenation (incl dataset)
%- separating robot from object

\subsection{Architecture}
\label{sec:architecture}
DistinctNet takes as input two images depicting the displacement of an object and otherwise static background.
This input pair is processed by the first two ResNet blocks in siamese fashion with shared weights.
A correlation layer then calculates the similarity between the two feature volumes to derive information on possible displacement, which is commonly done in disparity or optical flow estimation architectures (e.g. \cite{dosovitskiy2015flownet, ferrari_segstereo_2018}). 
Inspired by \cite{rocco_convolutional_2017} we normalize features before and after the correlation operation, and finally apply a \emph{ReLU} non-linearity.
The output thereof is concatenated with the two feature maps and channel-wise reduced
% (\emph{Conv2d} - \emph{Batchnorm} - \emph{ReLU}) 
to fit the input dimension of the following ResNet block. 
Finally, forwarding through the remaining DeepLabv3+ modules generates pixel-wise probabilities of foreground and background.
Additional output channels concatenated to the final layer of the network are utilized to predict different parts of the moving foreground like manipulator and object.

Furthermore, we experiment with \emph{Convolutional LSTM} (\emph{ConvLSTM}) layers \cite{shi_convolutional_nodate} after the ASPP module and in the Decoder which let us predict object and manipulator even if their motion between consecutive frames comes to a halt.
We investigate the performance of these recurrent layers in Sec.~\ref{sec:extreme_stop}.
Last but not least, we evaluate the placement of the correlation operation in our network in Sec. \ref{sec:ablation}, where we also consider employing a co-attention layer~\cite{lu_hierarchical_2016,lu_see_2019}.

%See Fig. \ref{fig:arch} for a complete overview of our architecture.
%Training details are summarized in Table \ref{tab:diffnet_training_settings}.




%\begin{table}[!ht]
%	\centering
%	\caption[Training settings]{Quantitative comparison of our method compared to three baseline approaches and \cite{florence2019self}; for a better overview we first list the joint objects. The right-most column shows results on semantic segmentation in a table top scene, where we use our automatically generated object masks as training data. Numbers in \textbf{bold} denote the best results on object-in-gripper segmentation.}
%	\vspace*{1mm}
%	\resizebox{\columnwidth}{!}{
%		\input{../tables/diffnet_training_settings}}
%	\label{tab:diffnet_training_settings}
%\end{table}

\subsection{Moving Object Segmentation}
\label{sec:moving_obj_seg}


We first train DistinctNet to learn a semantic agnostic representation of a moving object in front of static background. 
While there exist several segmentation datasets with moving items in a scene \cite{wang_cdnet_2014, perazzi_benchmark_2016, abu_alhaija_augmented_2018}, they are either limited to specific items, have multiple moving objects or additionally move the camera.
Consequently, we use BlenderProc~\cite{denninger_blenderproc_2019} to generate realistic-looking synthetic image pairs of static scenes with one random object in motion between two consecutive frames, which we explain in full detail in \mbox{Sec.~\ref{sec:dataset_fg}}.
The synthetic image pairs let the network effectively reason about an unknown moving object in an otherwise static scene.
%Training the model until convergence with a batch size of four takes roughly four days on a single Nvidia GeForce RTX 2080 Ti.

\subsection{Distinction between Manipulator and Grasped Object}

After training moving foreground estimation, DistinctNet is well suited to distinguish a moving manipulator without any grasped object from static background. 
Following the self-supervised paradigm these automatically generated masks are further used as training data, and we explain the respective details in Sec. \ref{sec:dataset_robobj}.
%The respective generation of this data is explained in \ref{sec:dataset_robobj}.
Importantly, the architecture of DistinctNet directly allows for fine-tuning on object-manipulator differentiation by increasing the number of output channels in the final layer.
%Instead of having to employ a second estimator, we simply add semantic channels to the output layer.
%Instead of having to employ a second estimator, we increase the number of output channels of the final layer.
Now, the network is capable of moving foreground segmentation as well as semantically interpreting and distinguishing moving parts into manipulator and object in the additional channels.


%To incorporate temporal information of previous frames we add a convolutional LSTM layer (ConvLSTM \todo{format} \todo{cite}) after the ASPP module, and replace every standard convolutional layer in the decoder with its LSTM counterpart.

%Finally, the decoder outputs a two channel map which, after a softmax operation, denotes the probability of a pixel belonging to moving foreground or static background.
%When fine-tuning on grasped object segmentation two additional channels are added for object and manipulator, respectively. 
%We provide detailed experimental results of the contribution of each architectural part in Section \todo{section}.




%Once trained on moving foreground segmentation we use DiffNet to automatically generate annotations of a moving manipulator in front of a static scene.

%Following previous work we use DiffNet to automatically generate segmentation masks of a moving robotic manipulator in front of static background.

%A major contribution of this work is to simultaneously optimize moving foreground and object-manipulator differentiation. 
%Given our architecture that is able to semantically differentiate moving foreground from static background, this can simply be achieved by adapting the last layer to output two additional channels for object and manipulator, and the model is fine-tuned with a multi-class binary cross entropy loss.

The semantic foreground separation can be pushed even further: 
Remarkably, it allows us to resolve the constraint on static background as we can denote an additional channel for all moving items other than the grasped object and manipulator.
%We believe that this enhances practical applicability of our approach since a completely static background cannot always be assured,
Our aim here is to enhance the practical applicability of our approach, given that a completely static background cannot always be assured.
%We believe that this tremendously improves the practical applicability of our method 
An experimental evaluation of this is given in Sec.~\ref{sec:garbage}.






==> related_work.tex <==
%For a self-supervised training data generation we briefly review related work for foreground segmentation to estimate a robot / joint robot-object mask, as well as methods that then separate the object from the manipulator.

We briefly discuss existing work on self-supervised object segmentation.
Additionally, we review methods that reason about correspondences between a pair of images.
Relevant to this work are also approaches which combine motion and semantic segmentation.

\subsection{Self-Supervised Grasped Object Segmentation}

A robot arm has initially been utilized for object segmentation by inducing motion in a static scene (e.g.~\cite{Fitzpatrick2003GroundingVT,schiebener_physical_2014,pathak_learning_2018, deng2020self}).
%\cite{} verify segmentation hypotheses by grasping the respective object.
To have more control over the object motion, grasping the respective item is a reasonable consequential step - however, it additionally requires distinguishing the object from the manipulator.
This can be addressed with the help of a 3D robot model which allows to isolate the object~\cite{krainin_manipulator_nodate,welke_autonomous_2010}. 
Browatzki~et~al.~\cite{browatzki_active_2012} employ a perception-driven object recognition framework where the robot itself controls the object views, and segment the item area with a GMM.
Instead, \cite{rocha_self-supervised_2019} propose a self-supervised approach for pixel-wise robot recognition:
By projecting a robot model onto the image plane and simultaneously optimizing a GrabCut-based cost function, segmentation labels of the robot arm are obtained.
Florence~et~al.~\cite{florence_robot-supervised_2020} build upon this framework and extend it to grasped object segmentation:
% and only registers manipulator coordinates in the camera frame.
They segment the foreground by projecting link positions of the robot into the camera frame which aids a graph-based depth segmentation followed by an additional refinement in RGB space.
%After a refinement in RGB space a foreground mask is obtained with the help of GrabCut.
With this approach they collect segmentation masks of the manipulator to learn a robot arm representation. 
%In an RGB-based refinement they fill all holes and perform morphological operations to compensate for depth sensor noise. This estimate is then refined to a final foreground mask using GrabCut.
%To differentiate robot arm from object they first collect training samples of solely the robot arm moving. Then, they paste these arms on random backgrounds together with an occluding object at the end effector position. With this training data they train a network on visible robot arm segmentation.
During inference they obtain a joint robot-object mask with the same foreground segmentation, and subtract the manipulator with help of the robot arm segmentation network.
%Yet, this adds the additional task of differencing object from manipulator in the visual sensor data.
%This can be addressed by knowledge of the 3D model of the robot
%- other related work: browatzki etc.
%- in contrast: no calibration etc., in contrast to ours: no postprocessing
In our previous work~\cite{boerdijk_self-supervised_2020} we alleviate the constraints of the aforementioned methods in form of precise camera calibration and additional sensor modalities by observing motion in a static scene, and learn a manipulator representation from thresholded optical flow only.
Excluding the manipulator estimation from the joint object-manipulator mask - again derived by motion - yields the final object mask.
%The pipeline performs regardless of the camera's placement and solely works with consecutive single RGB frames.

Yet, optical flow incorporates little semantic knowledge which requires additional post-processing. 
Moreover, none of the above approaches utilize a single, end-to-end trainable architecture.
%In this paper we rethink the utilization of motion for self-supervised object segmentation.
%Instead of a separate foreground and semantic estimator we combine both in a single architecture which does not require any post-processing.
%Our results show that semantic knowledge improves the agnostic segmentation by motion, and our pipeline performs better than our previous work without requiring any post-processing.


%Once the foreground is estimated, it remains to differentiate the manipulator from the grasped object. In a self-supervised scenario this is typically done by leveraging data derived from the foreground segmentation

\subsection{Exploring Correspondences between Images}

Finding dense correspondences between a pair of images is one of the fundamental tasks of computer vision.
Input pairs can be different views of a scene \cite{hosni_fast_2013, hirschmuller_stereo_2008}, consecutive video frames \cite{horn_determining_nodate, teed_raft_2020} or even an image pair depicting different instances of the same semantic class as in the case of semantic correspondence matching \cite{liu_sift_nodate, rocco_convolutional_2017, lee_sfnet_2019}.
We aim to segment moving objects from otherwise static background; hence we focus on the second category where change detection \cite{radke_image_2005} or background modeling \cite{bouwmans_subspace_2009} are fundamental algorithms.
%Constraints such as camera motion, non-static backgrounds or simply the abundance of enough change have soon let to an emerge of specific background modeling techniques.
Due to superior performance of neural networks in many image-related tasks, \emph{Convolutional Neural Networks} (\emph{CNNs}) have also been applied~\cite{bouwmans_deep_2019}. De~Jong~et~al.~\cite{de_jong_unsupervised_2019} target the problem of unsupervised change detection in satellite images and propose a siamese architecture with feature fusion by concatenation. Ru~et~al.~\cite{ru_multi-temporal_2020} merge CNN features with a canonical correlation analysis to detect semantic changes in urban regions.
%, and we refer the reader to \cite{bouwmans_deep_2019} for a detailed overview.

Optical flow is another way of obtaining pixel-wise correspondences between images, and current state-of-the-art approaches usually employ correlation in deep feature space to obtain a dense flow map (e.g. \cite{fischer_flownet_2015, hui_liteflownet_2018, teed_raft_2020}).

Since the rise of attention \cite{vaswani_attention_2017} several works explore differences between two data features with so-called \emph{co-attention}. 
This has initially been studied for vision-language tasks \cite{lu_hierarchical_2016, wang_learning_nodate}, but already has been applied successfully to the image domain: 
Lu et al. \cite{lu_see_2019} use co-attention for semantic video segmentation and achieve state-of-the-art performance for unsupervised video segmentation on DAVIS~\cite{perazzi_benchmark_2016} at their time of release. 

%Our work is inspired by these formulations, and we learn to segment agnostic moving objects from static background to segment a moving manipulator (optionally equipped with an object).

%Inspired by semantic alignment (e.g. \cite{endtoend_rocco, }), where the task is to find correspondences between 

%While geometric matching is a particularly related field 
%A particularly related problem is semantic correspondence, 

\subsection{Combination of Motion and Segmentation}
\label{sec:rl_combination}
Many dense correspondence estimators have successfully been coupled with specific semantic knowledge.
For instance, Cioppa~et~al.~\cite{cioppa_real-time_2020} propose a background modeling algorithm that is updated with predictions of a semantic segmentation network which has learned important object-related features and aids the overall pipeline.
%This second predictor has learned important features of specific object classes and aids the overall pipeline.
%However, the respective network is pre-trained to have knowledge on specific classes.
Similar work exist for optical flow estimation: \cite{sevilla-lara_optical_2016} apply prior knowledge on a pixel's motion by defining different motion models for specific semantic regions. 
Bai~et~al.~\cite{bai_exploiting_2016} segment potentially moving objects, estimate flow individually and merge the predictions with background motion to improve accuracy.
In~\cite{bideau_best_2018}, classical geometric knowledge of moving objects is combined with high-level semantic image understanding in order to improve performance.
Hur~et~al.~\cite{hur_joint_2016} utilize flow to enforce temporal segmentation consistency, and simultaneously pose epipolar constraints inferred from semantic information on the motion estimation. 
Cheng~et~al.~\cite{cheng_segflow_2017} propose to jointly predict optical flow and semantic segmentation masks by employing a two stream approach, while \cite{tokmakov2019learning, jain2017fusionseg} segment moving objects by employing a specific motion and appearance network.
%More general formulations jointly estimate optical flow and semantic segmentation in a two stream approach , hur_joint_2016}.
%\cite{cheng_segflow_2017} pair ResNet-101 and FlowNetS to a two-branch architecture and jointly predict optical flow and segmentation. 
%Similarly, \cite{dave_towards} employ a two stream model and merge motion and appearance in feature space. -> not in here as they require flow as input
%\todo{Test their pretrained network on foreground estimation, add params: https://github.com/JingchunCheng/SegFlow}
%\cite{hur_joint_2016} jointly train optical flow estimation and semantic segmentation.

Nevertheless, the current best performing methods on the Kitti Optical Flow Benchmark \cite{noauthor_kitti_nodate} solely estimate optical flow. 
Concurrently we observe that flow architectures usually differ from semantic segmentation networks, as features for each task are extracted differently.
% - usually, flow architectures are much shallower to reduce computational cost for correlation estimation.
Moreover, we argue that optical flow itself over-complicates moving foreground extraction for object segmentation: for a respective binary mask it is solely interesting whether an object moves or not; direction and magnitude of each pixel do not yield any benefits.

%In our previous work \cite{boerdijk_self-supervised_2020} we investigate thresholded optical flow as foreground segmentation.
%While this is an elegant solution it over-complicates the problem at hand:
%While thresholded optical flow can be capable of estimating strong segmentation masks of moving objects the task itself is overcomplicated.
%Rather than knowing to which spatial position an object moves, we are only interested in a binary prediction of whether it moves at all or not.
%Our decision to refrain from utilizing optical flow predictors is further motivated by the fact that flow architectures (e.g. Liteflownet, Raft, FlowNet) typically differ from semantic ones (e.g. Deeplab).
%Due to multiple correlation operations in feature space the respective feature maps 

%In this paper we rethink the utilization of motion for self-supervised object segmentation.
%Instead of a separate foreground and semantic estimator we combine both in a single architecture which does not require any post-processing.
%Our results show that semantic knowledge improves the agnostic segmentation by motion, and our pipeline performs better than our previous work without requiring any post-processing.
Consequently, we rethink the utilization of motion in our self-supervised object segmentation pipeline. 
We propose an architecture that can efficiently estimate dense correspondences between features, and is additionally capable of incorporating specific semantic attributes.
%, and can hence be fine-tuned on distinguishing manipulator from object.
In contrast to previous self-supervised grasped object segmentation approaches our framework consists of a single network that is trainable end-to-end, and does not require any post-processing.
%based on a semantic segmentation network. 
%We add a single global correlation layer to investigate differences between an input pair of images in feature space.
\begin{figure*}[!ht]
	\vspace{3mm}
	\centering
	\captionsetup{width=\linewidth}
	\includegraphics[width=0.98\linewidth]{../figures/diffnet_architecture/arch_final.png}
	\caption{Architectural overview (best viewed magnified). \emph{DistinctNet} can be trained on moving foreground segmentation  (left image cuts; green border) and afterwards fine-tuned on semantically distinguishing foreground into manipulator, object and optional other semantic classes such as moving background objects (right image cuts; blue border). Dashed lines denote optional recurrent layers. Note that the last three output channels (here depicting manipulator, object and a moving background object) are only available during fine-tuning.}
	\label{fig:arch}
\end{figure*}%

%What further motivates not integrating a semantic branch into a flow network is that current state of the art flow predictors abstain from additionally predict semantic masks.


%sum:
%- methods are not differentialbe, consist of multiple frameworks, pretrained, specific semantic classes



%can be especially difficult due to lighting changes, camera motion or non-static backgrounds.
%Often, the problem at hand is not any more solvable with basic change detection \cite{radke_image_2005}, but more sophisticated background modeling algorithms are employed.

%-- change detection
%Basic / naive change detection: image differences
%Has also been tried with cnns


% (we dont want that: semantic net has to be trained, classes have to be known, no way of directly optimizing)
%While they achieve state-of-the-art performance on CDNet2014, the approach relies on a pre-trained semantic segmentation network that has already learned specific classes.




%\subsubsection{Semantic Foreground Segmentation}










%In this work, we derive a binary segmentation mask of an object moving between two consecutive frames with a single correlation operation in feature space. This results in a faster inference time and less parameters than [co-attention], and importantly also better results for our problem.

%the speed vectors are not necessarily required to derive a binary segmentation mask of moving objects. In this work, we abstain from solving the orientation and magnitude of motion for each pixel, and instead directly solve the much simpler task by asking \emph{Does this pixel move or not?}
%To this end, we learn to semantically identify a moving object from static background from synthetic data only.

%Motion 

%- automatic training data generation

%	why our approach is necessary
%		mainly: no object models available

%- foreground segmentation / differences between images (also: motion)

%	mention camera jitter, noise etc.
%	mention prominent datasets that target evaluation of these issues?
%		caveat: why dont we evaluate our method on this?
%		e.g. CDNet2014: moving cameras, background noise etc.

%\subsubsection{Separating Object from Manipulator}



%Our architecture is especially motivated by the thought whether we need speed vectors and magnitude etc.

%In our previous work [ours] we 





%- attention / co-attention




%Semantic segmentation + optical flow




%Differences to ours:
%- dont need speed vectors
%- only one object that moves
%- most other network architectures that output both jointly are too heavyweight
%- we want to train end to end, so we need a net that can estimate differences based on semantic features
%- no current methods that jointly estimate flow and segmentation together on leaderboard of kitti
%- mention that motion is a strong prior for foreground estimation
%
%
%- differences to florence, browatzki: no ego perspective!






%- joint robot-object learning / how to detect object?






%Differences to ours old:
%- no postprocessing
%- pre-trained model universally applicable

%last sentence: say stuff about architecture, general setting (then skip part in method!)


==> setup.tex <==
%We use the same recording setup as in our previous approach and refer the reader to \todo{cite} for a detailed overview.
%We summarize the most important aspects below, and in detail discuss differences.
\subsection{Training Datasets}
\subsubsection{Moving Object Segmentation}
\label{sec:dataset_fg}
With BlenderProc \cite{denninger_blenderproc_2019} we sample a camera position inside a random room of the SunCG dataset \cite{song_semantic_2016}, select an object inside the camera's view and render ten frames while we randomly shift and rotate the respective item. % (see Fig. \ref{fig:dataset}).
We repeat this procedure to obtain 5,000 sequences of random moving objects in a static scene.
DistinctNet is then trained on moving object segmentation (90/10 train/val split), where an input pair consists of two images of one sequence.
%Consequently, one epoch consists of 50,000 forward passes.
%We use 90\% as training data and validate performance on the remaining 500 sequences.
% with standard Cross Entropy Loss and AdamW \todo{cite} optimizer.
%Following widely adopted practice \todo{cite} we set the learning rate to 1e-3 and reduce it by a factor of 0.1 for all backbone parameters (including the reduction layer).
%We augment each image independently with random channel shuffling, color jitter and Gaussian noise and blur. 
%For exact parameters please see the Appendix. \todo{appendix}

\subsubsection{Fine-Tuning on Robot-Object Segmentation}
\label{sec:dataset_robobj}
The training data for this task should consist of moving robotic arms with a grasped object in front of random, stationary background.
Hence, for each training pair we duplicate a random image of the MS COCO dataset \cite{lin_microsoft_2015} to emulate diverse static background. 
We further sample two random robot arms (one for each image) and augment the presence of an object at the gripper's end effector with an occluding object.
As in our previous work \cite{boerdijk_self-supervised_2020} we derive the corresponding object pasting spots by opening and closing the gripper at static position and once again segment moving foreground with DistinctNet.
As occluders we use random objects from the ShapeNet dataset \cite{chang_shapenet_2015} whose orientation, texture and lighting can be realistically simulated with BlenderProc.
Note that while we use the same object for both images in a training pair its orientation can be different.
In total we generate 50,000 sample pairs (90/10 train/val split).

During training we separately augment each image with Gaussian noise, and add random color jitter for both the whole image as well as the occluding object. 
Additionally, to cope with pasting artifacts which can present a simple shortcut to the network during learning \cite{dwibedi_cut_2017}, we apply a median blur on the full image.

For our validation set we do not cut out robot masks, but directly paste objects on the test backgrounds.
We do not augment these images to verify the generalization capability onto novel environments and objects.

\subsection{Implementation Details}
\label{sec:implementation_details}
The global correlation layer restricts us to a fixed input size, and we consequently resize images to 414x746~pixels.
All experiments are conducted on a single Nvidia GeForce RTX 2080 Ti. 
We use AdamW \cite{loshchilov_decoupled_2019} as optimizer with a weight decay of 0.01.
For moving object segmentation we use standard cross entropy loss and set the learning rate to 1e-3 with a reduction to 1e-4 for all ResNet layers.
When fine-tuning on semantic classes we freeze all encoder weights before the correlation operation and train with a multi-class binary cross entropy loss combined with a reduced learning rate of 1e-4 for all trainable parameters.
Training takes roughly four (moving object segmentation) and three (semantic finetuning) days with a batch size of 2 on a single Nvidia GeForce RTX 2080.



\subsection{Recording Setup and Test Dataset}
\label{sec:dataset_test}
Our robot arm is a KUKA LBR4+ %\cite{methods_lbr_url} 
on a linear axis employed with a Robotiq 2F-85 two-finger gripper. %\cite{methods_gripper_url}.
All data is recorded with a ZED stereo sensor. %\cite{zedstereo}.

%\subsection{Test Dataset}

We use the same 15 YCB object recordings as in our previous work (301 images per object), and refer the reader to~\cite{boerdijk_self-supervised_2020} for a detailed recording protocol.
45 images per object already contain manually annotated segmentation masks, and we additionally label the respective robot arms for a complete evaluation of foreground, robot and object.

%\subsection{Baselines}
%
%We re-implement basic change detection \cite{} to additionally provide performance details on foreground extraction and robot segmentation masks.
%
%We create a binary change detection mask by using Otsu thresholding \todo{cite} on the absolute pixel-wise difference of two images.
%We obtain a joint manipulator-object mask with i
%
%For completion we also provide an optical flow based change detection baseline with RAFT.
%
%DiffNet does not need any form of post-processing to produce object masks of satisfactory quality. For a fair comparison we therefore do not employ any post-processing on any of these baselines.


%We use the data from ours.
%
%For better comparison and evaluation of our method we additionally annotate robot arms and the moving foreground. We re-implement the baselines of ours old with a few modifications for better comparison:
%For equal comparison we do not employ any post-processing to ensure generalization capability on any environments.
%
%- Change Detection: otsu thresholding
%- optical flow backbone: raft (of cd, ours reimplemented)
%
%In contrast to ours old, 
%
%\subsection{Datasets}
%
%\subsection{Training Details}
%
%We train with cross entropy loss and AdamW \todo{cite} optimizer. 
%The learning rate is set to 1e-3, and, following widely adopted practice \todo{cite}, reduced by 0.1 for the backbone. 
%We use 45,000 image pairs as training and 5,000 as validation data, respectively.
%
%The model is initially trained without the ConvLSTM layers on single image pairs only for \todo{epochs}. 
%Afterwards, the decoder is fine-tuned together with the recurrent layers on image sequences of length 10 for \todo{epochs, lr; finetune res3, res4 too?} while the backbone and ASPP weights are frozen.
%Then, the model is able to efficiently separate moving from static objects from a sequence of images.
%
%For the grasped object segmentation the weights of the encoder are frozen, and all other layers are trained with a reduced learning rate of 1e-4 for \todo{epochs}.
%
%
%\subsubsection{Moving Object Segmentation}
%
%
%
%\subsubsection{Grasped Object Segmentation}
%
%also: testset!
%
%
%
%
%
%
%\subsection{Visible Manipulator Segmentation}
%
%- either pasting or multihead self-attention
%
%\subsection{Differentiation between Manipulator and Object}
%
%- either paste
%- or multihead self-attention
%
%
%
%
%
%
%
%\subsection{title}
%
%Following our previous work
%
%\subsection{Baselines}
%
%- divide between foreground estimation and robot-object differentiation?
%
%foreground estimation baselines
%- from previous: change detection (rgb / of space)
%- re-implement previous with RAFT
%- of / seg paper: [SegFlow/cheng,tsai]
%- bg modeling paper: [real-time semantic/cioppa]
%
%\subsection{Test Set and Metrics}
%
%- foreground estimation: manually annotated robot arms, random subset
%- grasped object segmentation: manually annotated ycb objects
%
%- downstream tasks: semantic segmentation (table top dataset), detection (table top dataset), 3d reconstruction?
%
%- metrics: standard mean iou, f1 score


